Analysing kinematic data from recreational runners using functional data analysis

We present a multivariate functional mixed effects model for kinematic data from a large number of recreational runners. The runners' sagittal plane hip and knee angles are modelled jointly as a bivariate function with random effects functions used to account for the dependence among measurements from either side of the body. The model is fitted by first applying multivariate functional principal component analysis (mv-FPCA) and then modelling the mv-FPCA scores using scalar linear mixed effects models. Simulation and bootstrap approaches are introduced to construct simultaneous confidence bands for the fixed effects functions, and covariance functions are reconstructed to summarise the variability structure in the data and thoroughly investigate the suitability of the proposed model. In our scientific application, we observe a statistically significant effect of running speed on both the hip and knee angles. We also observe strong within-subject correlations, reflecting the highly idiosyncratic nature of running technique. Our approach is more generally applicable to modelling multiple streams of smooth kinematic or kinetic data measured repeatedly for multiple subjects in complex experimental designs.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> main/simulation.tex <==
\section{Simulation Study} \label{sec:bfmm-simulation}

We perform a short simulation study to demonstrate the properties of our method in two scenarios. The first scenario assumes that the fixed effects, random effects and random error terms are generated by the same bivariate FPC basis, which means our proposed model is correctly specified. In the second scenario, a different bivariate basis is used for the fixed effects, random effects and random error terms, in which case our proposed model is an approximation.

To liken the simulation setting to the real data application, we use empirical parameter estimates to generate the data. We generate data from $N = 280$ subjects with two bivariate functional observations each to mirror our study design, i.e., hip and knee angles measured on both sides of the body for each subject. For each subject, we generate two covariates -- a continuous self-selected running speed variable and a binary sex variable; both covariates were included in our final model for the real data analysis. Observations are simulated according to the model
$$
\mathbf{y}_{ij} (t) = \boldsymbol{\beta}_0 (t) + \boldbeta_1 (t) \times\text{sex}_i + \boldbeta_2 (t) \times \text{speed}_i + \boldut + \boldepst,
$$
for $i = 1,\dots, 280, \ j = 1, 2, \ t \in [0, 100]$ and $\text{sex}_i \in \{0, 1\}$. This is a version of model \eqref{FMM} with $A = 2$, we have simplified the model to have only two fixed effect parameters to keep the simulation and presentation of results concise.

In both scenarios, we use empirical estimates for the fixed effects functions $\boldbeta_0 (t)$, $\boldbeta_1 (t)$ and $\boldbeta_2 (t)$, and use 13 bivariate basis functions to generate the model terms because 13 bivariate FPCs explained $99\%$ of the variability in the real data application. For the first scenario, we use the same basis of 13 empirical bivariate FPCs to generate $\boldut$ and $\boldepst$. In the second scenario, we use 13 bivariate Fourier basis functions for $\boldut$ and 13 bivariate polynomial basis functions for $\boldepst$ \parencite{happ-kurz_object-oriented_2020}. In both scenarios, we draw the basis coefficients of the functional random intercepts and functional random errors from a multivariate Gaussian distribution with a diagonal covariance matrix, and use empirical estimates for the coefficient variances (i.e., $\widehat{q}_k$ and $\widehat{s}_k$, $k=1, \dots 13$ from our fitted model). Figure \ref{fig:simulated-data} shows 10 simulated bivariate functional observations from both data-generating scenarios.


\begin{figure}[!htbp]
    \centering
    \includegraphics[width = 1\textwidth,page=2]{figures/figures.pdf}
    \caption{10 simulated bivariate functional observations from the first and second simulation scenarios.}
    \label{fig:simulated-data}
\end{figure}


We evaluate each fixed effect estimate in terms of integrated squared error (ISE), defined as 
$$
\text{ISE}(\widehat{\boldsymbol{\beta}}_a) = \int_0^{100} \left\{\widehat{\beta}^{(hip)}_a (t) - \beta^{(hip)}_a (t)\right\}^2 \mathrm{d}t + 
\int_0^{100} \left\{\widehat{\beta}^{(knee)}_a (t) - \beta^{(knee)}_a (t)\right\}^2 \mathrm{d}t,
$$
for $a = 0, 1, 2$. We consider the coverage probabilities of the pointwise confidence intervals and simultaneous confidence bands. The matrix-valued covariances of the bivariate functional random intercepts and bivariate functional random errors are also assessed in terms of ISE
$$
\text{ISE}(\widehat{\mathbf{Q}}) = \int_0^{100}  \int_0^{100}  \sum_{p \in \{\text{hip, knee}\}} \sum_{p' \in \{\text{hip, knee}\}} \left\{\widehat{Q}^{(pp')}(t, t') - Q^{(pp')}(t, t')\right\}^2 \mathrm{d} t \mathrm{d}t',
$$
with the $\text{ISE}$ for $\widehat{\mathbf{S}}$ defined similarly. The ICC and the number of bivariate FPCs retained are also examined. For both scenarios, we generate 500 simulated datasets. The mv-FPCA truncation is fixed at $99.99\%$, $1000$ bootstrap replications are used, \num{10000} multivariate Gaussian samples are drawn for the confidence bands and a nominal level of $95\%$ is used for the confidence intervals.

Figure \ref{fig:simulation-results} shows the estimation results. There is little difference in fixed effects estimation between the two scenarios (top panel). The ISE values for $\boldsymbol{\beta}_1 (t)$ are larger than those for $\boldsymbol{\beta}_2 (t)$, simply because of a smaller signal-to-noise ratio for this effect. For the random-effect and random-error covariances (middle panel), estimation is substantially better under Scenario 1 than under Scenario 2. The model estimates (boxes with a black outline) are much closer to the unstructured estimates, (boxes with a grey outline) under Scenario 1. The ICC is estimated similarly and centred on the true value in both scenarios (bottom panel). To summarise, the fixed effects functions and ICC are estimated comparably well in both scenarios. However, when the model is incorrectly specified in Scenario 2 (i.e., different bases are used for the fixed effect, random-intercept and random-error functions), estimation quality of the covariance structures is reduced significantly. As shown empirically in our data application in Section \ref{sec:bfmm-results}, this is because of the restriction of the diagonal assumption for $\mathbf{Q}^*$ and $\mathbf{S}^*$ -- correlation (in the random-intercept and random-error terms) between FPCs is required to fully reconstruct the covariance functions.

Table \ref{tab:coverage-probs} contains the coverage probability estimates from the simulation along with Monte Carlo standard errors, which quantify simulation uncertainty due to the finite number of simulation repetitions \parencite{morris_using_2019}. Pointwise and simultaneous coverage probabilities are close to nominal and performance of the bootstrap and Wald methods is comparable in both scenarios. This indicates that although the covariance structures are reconstructed with error in Scenario 2, they still allow for fast approximate uncertainty estimates that work reasonably well to be constructed. It should be noted that the reported pointwise coverage is an ``across the function" average -- it is averaged across the functional domain and across the two dimensions of the bivariate function. Additional analysis, contained in Appendix \ref{additional-simulation-results}, reveals that the Wald intervals tend to over- and under-cover at different points along the function in Scenario 2. In comparison, the pointwise coverage of the bootstrap intervals is stable and may be preferred.

{
\begin{table}[]
\centering
\begin{tabular}{cccccc}
\hline
\multirow{2}{*}{\textbf{Method}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Coverage\\ Type\end{tabular}}} &
  \multirow{2}{*}{\textbf{Scenario}} &
  \multicolumn{3}{c}{\textbf{Parameter}} \\ \cline{4-6} 
                           &                               &   & $\boldsymbol{\beta}_0(t)$ & $\boldsymbol{\beta}_1(t)$ &
                           $\boldsymbol{\beta}_2(t)$ \\ \hline
\multirow{4}{*}{Wald}      & \multirow{2}{*}{Pointwise}    & 1 & 0.95 (0.01)  & 0.96 (0.01)  & 0.96 (0.01) \\
                           &                               & 2 & 0.94 (0.01)  & 0.95 (0.01)  & 0.95 (0.01)  \\ \cline{2-3}
                           & \multirow{2}{*}{Simultaneous} & 1 & 0.94 (0.01)  & 0.96 (0.01)  & 0.96 (0.01)  \\
                           &                               & 2 & 0.92 (0.01)  & 0.95 (0.01)  & 0.94 (0.01)  \\ \cline{1-3}
\multirow{4}{*}{Bootstrap} & \multirow{2}{*}{Pointwise}    & 1 & 0.95 (0.01)  & 0.95 (0.01)  & 0.95 (0.01)  \\
                           &                               & 2 & 0.95 (0.01)  & 0.95 (0.01)  & 0.95 (0.01)  \\ \cline{2-3}
                           & \multirow{2}{*}{Simultaneous} & 1 & 0.92 (0.01)  & 0.95 (0.01)  & 0.94 (0.01)  \\
                           &                               & 2 & 0.93 (0.01)  & 0.96 (0.01)  & 0.94 (0.01)  \\ \hline
\end{tabular}
\caption{Coverage probability estimates of the $95\%$ pointwise confidence intervals and simultaneous confidence bands obtained from the simulation. Estimated Monte Carlo standard errors are shown in brackets to quantify simulation uncertainty. The pointwise coverage probabilities have been averaged across the functional domain and across dimensions of the bivariate function.}
\label{tab:coverage-probs}
\end{table}
}


\begin{figure}[!htbp]
    \centering
    \includegraphics[width = 1\textwidth,page=3]{figures/figures.pdf}
    \caption{Estimation results from the simulation study under the two data-generating scenarios (1 = red, 2 = turquoise). \textbf{Top panel}: The ISE values for the fixed effects functions $\boldsymbol{\beta}_1 (t)$ (left panel) and $\boldsymbol{\beta}_2 (t)$ (right panel). \textbf{Middle panel}: The ISE values for the random-effects covariance function $\mathbf{Q}(t, t')$ (left panel) and the random-error covariance function $\mathbf{S}(t, t')$ (right panel). The boxplots with black trimming show the model estimates and are presented next to unstructured estimates shown by the boxes with grey trimming. \textbf{Bottom panel}: The ICC estimates with the true ICC value overlaid as a solid horizontal black line.}
    \label{fig:simulation-results}
\end{figure}

Empirical investigations on our real dataset to compare our proposed approach with existing approaches for univariate and multivariate functional mixed effects models are contained in Appendix \ref{app:comparisons}.
